Differentiable Manifold Reconstruction for Point Cloud Denoising

3D point clouds are often perturbed by noise due to the inherent limitation of acquisition equipments, which obstructs downstream tasks such as surface reconstruction, rendering and so on. Previous works mostly infer the displacement of noisy points from the underlying surface, which however are not designated to recover the surface explicitly and may lead to sub-optimal denoising results. To this end, we propose to learn the underlying manifold of a noisy point cloud from differentiably subsampled points with trivial noise perturbation and their embedded neighborhood feature, aiming to capture intrinsic structures in point clouds. Specifically, we present an autoencoder-like neural network. The encoder learns both local and non-local feature representations of each point, and then samples points with low noise via an adaptive differentiable pooling operation. Afterwards, the decoder infers the underlying manifold by transforming each sampled point along with the embedded feature of its neighborhood to a local surface centered around the point. By resampling on the reconstructed manifold, we obtain a denoised point cloud. Further, we design an unsupervised training loss, so that our network can be trained in either an unsupervised or supervised fashion. Experiments show that our method significantly outperforms state-of-the-art denoising methods under both synthetic noise and real world noise. The code and data are available at https://github.com/luost26/DMRDenoise

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> old/3.4-loss.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Dual Loss Functions}
To optimize the entire denoising process, we consider {\it dual loss} to measure the quality of both the subsampling and final point cloud reconstruction. 
That is, we have two loss functions, including 
1) a loss function $\mathcal{L}_{\mathrm{sample}}$ to quantify the distance between the subsampled and pre-filtered set $\hat{\S}$ and the ground truth point cloud $\P_\mathrm{gt}$, which explicitly reduces the noise in $\hat{\S}$ but is not required for the convergence of the training; 
2) a loss function $\mathcal{L}_{\mathrm{rec}}$ to quantify the distance between the finally reconstructed point cloud $\tP$ and the ground truth $\P_\mathrm{gt}$. 

Formally, our network can be trained end-to-end by minimizing 
\begin{equation}
    \min_{\Theta} \mathcal{L}_{\mathrm{sample}} + \mathcal{L}_{\mathrm{rec}},
\end{equation}
where $\Theta$ denotes the learnable parameters in the network.

We choose the Chamfer distance (CD) \cite{fan2017pointsetgen} as $\mathcal{L}_{\mathrm{sample}}$, since $\hat{\S}$ and $\P_\mathrm{gt}$ exhibit different number of points, \ie, $|\hat{\S}| < |\P_\mathrm{gt}|$. It is defined as
\begin{equation}
\label{eq:cd_train}
\mathcal{L}_{\mathrm{sample}} = \mathcal{L}_{\mathrm{CD}}(\hat{\S},\P_\mathrm{gt})= \frac{1}{\left|\hat{\S}\right|} \sum_{\p \in \hat{\S}} \min _{\q \in \P_\mathrm{gt}}\| \p - \q\|_2^2+\frac{1}{\left|\P_\mathrm{gt}\right|} \sum_{\q \in \P_\mathrm{gt}} \min _{\p \in \hat{\S}}\| \q - \p\|_2^2.
\end{equation}
This loss term improves the denoising quality by explicitly optimizing the sampled and pre-filtered set $\hat{\S}$, but is optional for the network training. 
In particular, this loss is not adopted when the network is trained in an unsupervised manner. 

$\mathcal{L}_{\mathrm{rec}}$ can be supervised or unsupervised, which are discussed below. 

\textbf{Supervised} $\mathcal{L}_{\mathrm{rec}}$.
% Our network takes noisy point clouds $\P$ as input and produces cleaned point clouds $\tP$. Hence, it is straightforward to utilize a loss function that measures the similarity between $\tP$ and the noiseless (ground truth) point cloud, denoted as $\P_\mathrm{gt}$. 
We choose the Earth Mover's distance (EMD) \cite{fan2017pointsetgen} as the supervised loss of $\mathcal{L}_{\mathrm{rec}}$, which is shown superior to the Chamfer distance in terms of the visual quality \cite{liu2019morphing, achlioptas2018learning}. 
The Earth Mover's distance is defined when two point clouds have the {\it same} number of points. 
Fortunately, the denoising task naturally satisfies this requirement. 
The EMD loss measuring the distance between the denoised point cloud $\tP$ and the ground truth point cloud $\P_\mathrm{gt}$ is given by:
\begin{equation}
\mathcal{L}_{\mathrm{rec}}=\mathcal{L}_{\mathrm{EMD}}\left(\tP, \P_\mathrm{gt}\right)=\min _{\varphi: \tP \rightarrow \P_\mathrm{gt}} \frac{1}{N} \sum_{\p \in \tP}\|\p-\varphi(\p)\|_{2}^2
\end{equation}
where $N = |\tP| = |\P_\mathrm{gt}|$, and $\varphi$ is a bijection.

Note that, previous works on denoising \cite{PCN2020, TotalDenoising2019} often suffer from the clustering effect of points, which is alleviated by introducing a repulsion loss. 
Our architecture does not suffer from this problem thanks to the one-to-one correspondence of points in $\mathcal{L}_\mathrm{EMD}$.
%Assuming the loss of our network has converged to an acceptable minumum, where $\mathcal{L}_\mathrm{EMD}$ is low, the output point cloud will not collapse around a single position, otherwise, $\mathcal{L}_\mathrm{EMD}$ will be high. However, if a non-symmetric Chamfer distance is used, like \cite{PCN2020} does, this situation might happen. As for the upsampling process, as observed in \cite{PPPU2019}, the upsampled points are not likely to gather too close to the original point, since the points are sampled from a manifold.
\newline

\noindent\textbf{Unsupervised} $\mathcal{L}_{\mathrm{rec}}$. 
Our network can also be trained in an unsupervised fashion. 
Leveraging an unsupervised denoising loss in \cite{TotalDenoising2019}, we design an unsupervised loss tailored for our manifold reconstruction based denoising.  
The key observation is that points with a denser neighborhood are closer to the underlying clean surface, which may be regarded as ground truth points for training a denoiser. 

In \cite{TotalDenoising2019}, the unsupervised denoising loss is defined as 
\begin{equation}
\mathcal{L}_{\mathrm{U}} = \frac{1}{N} \sum_{i=1}^{N} \mathbb{E}_{\q \sim P(\q | \p_i)} \| f(\p_i) - \q \|,
\end{equation}
where $P(\q|\p_i)$ is a prior capturing the probability that a point $\q$ from the noisy point cloud is the underlying clean point of the given $\p_i$ in the noisy point cloud.
Empirically, $P(\q|\p_i)$ is defined as $ P(\q|\p_i) \propto \exp ( - \frac{\| \q - \p_i \|_2^2}{2\sigma^2} )$, so that sampling points from the noisy input point cloud $\P$ according to $P(\q|\p_i)$ produces points that are closer to the underlying clean surface with high probability \cite{TotalDenoising2019}.
$f(\cdot)$ represents the denoiser that maps a noisy point $\p_i$ to a denoised point $\q_i$. It is a bijection between the noisy point cloud $\P$ and the output point cloud $\tP$. 

This bijection can be naturally established in previous deep-learning based denoising methods such as PointCleanNet \cite{PCN2020}, Total Denoising \cite{TotalDenoising2019} \etc, because these methods predict the displacement of each point. 
However, there is no natural one-to-one correspondence between $\P$ and $\tP$ in our method based on patch manifolds. 
Hence, we seek to construct one by
\begin{equation}
f=\arg\min _{f: \P \rightarrow \tP} \sum_{\p \in \P}\|f(\p) - \p\|_{2}.
\end{equation}

It has to be noted that, since the aforementioned loss term $\mathcal{L}_\mathrm{sample}$ requires the supervision of ground truth data, we will disable the term $\mathcal{L}_\mathrm{sample}$ and only use the unsupervised $\mathcal{L}_\mathrm{U}$ in the setting of unsupervised training.

